Time Does Tell: Self-Supervised Time-Tuning of Dense Image Representations

Spatially dense self-supervised learning is a rapidly growing problem domain with promising applications for unsupervised segmentation and pretraining for dense downstream tasks. Despite the abundance of temporal data in the form of videos, this information-rich source has been largely overlooked. Our paper aims to address this gap by proposing a novel approach that incorporates temporal consistency in dense self-supervised learning. While methods designed solely for images face difficulties in achieving even the same performance on videos, our method improves not only the representation quality for videos-but also images. Our approach, which we call time-tuning, starts from image-pretrained models and fine-tunes them with a novel self-supervised temporal-alignment clustering loss on unlabeled videos. This effectively facilitates the transfer of high-level information from videos to image representations. Time-tuning improves the state-of-the-art by 8-10% for unsupervised semantic segmentation on videos and matches it for images. We believe this method paves the way for further self-supervised scaling by leveraging the abundant availability of videos. The implementation can be found here : https://github.com/SMSD75/Timetuning

==> _old01_introduction.tex <==
\section{Introduction}
Large-scale training of visual representations using vision-language alignment~\cite{radford2021learning, jia2021scaling} or self-supervision~\cite{chen2020simple, goyal2021self, caron2021emerging} has demonstrated an enormous potential in terms of its emergent few- and zero-shot capabilities with increased robustness. Yet, these models have almost solely been trained on image data, despite the ubiquity and importance of video for tasks ranging from action recognition~\cite{kay2017kinetics} to understanding causality~\cite{lippe2022icitris, brehmer2022weakly}.
While previous methods have shown that adaptation of image models to the video domain is possible by finetuning~\cite{luo2022clip4clip, bain2021frozen} or adaptation~\cite{ju2021prompting}, the converse of learning meaningful information \textit{from videos for images}, like we do in this paper, have remained a key challenge.

Some works~\cite{gordon2020watching, kipf2021conditional} have attempted to leverage the passage of time 
as a type of image augmentation, or as a video learning signal~\cite{wei2018learning, ghodrati2018video}, however these works have generally reported reduced performances even when comparing to simple image based pretraining methods. 
As videos should strictly contain more information than the sum of its image parts, it seems that current video learning methods are simply not well-suited for learning modality-generalizable representations. In this work, we take inspiration from the recent progress in self-supervised learning of dense representations from images and in particular methods that conduct unsupervised object segmentation~\cite{van2021unsupervised, ziegler2022self, hamilton2022unsupervised, henaff2021efficient}. These generally train or finetune models using spatially dense losses, and in so doing achieve strong performances, especially when starting from image-level pretrained models such as DINO~\cite{caron2021emerging}. 
Motivated by this, the research question this paper addresses is the following: starting from image-pretrained models, how can we finetune these using videos in a way that benefits their dense representation capabilities?

\begin{figure*}[!t]
    \centering
    \includegraphics[width=2.0\columnwidth]{Images/TimeT.pdf}
    \caption{\textbf{\methodname~overview.} We conduct self-supervised video semantic segmentation by tuning image-pretrained models with temporal information from videos. \textbf{(a)}: Our general pipeline of adapting an image-pretrained ViT transformer on video data using our dense clustering loss. \textbf{(b)}: Detailed view into our Feature Forwarder module that is used for aligning cluster-maps from past frames to logit-features of future ones. Our method obtains state-of-the-art unsupervised semantic segmentation performances on videos \textit{and} images. }
    \label{fig:schematic}
\end{figure*}




Compared to the image domain, where crops and their locations can be used as dense signals to ensure spatial consistency~\cite{caron2020unsupervised, ziegler2022self}, such an explicit signal does not exist when moving to videos: when comparing two frames with each other, it is not immediately clear which pixels should retain similar embeddings and which should not, due to possible object, camera and background motion.

To this end, we introduce the Feature Forwarder (\textsc{FF}) module.
The \textsc{FF} leverages the good tracking performance of pretrained image models and allows us to infuse the model with temporal consistency. 
On top of this, we introduce a temporally dense clustering module, for which we adapt an online clustering framework~\cite{caron2020unsupervised} based on optimal-transport. 
Using these two components and starting from image-pretrained features, our proposed method allows \textit{timetuning} (\methodabbrev) the dense representation in a self-supervised manner.
This achieves state-of-the-art performances not only for the task of unsupervised semantic segmentation of videos, but also for \textit{image} semantic segmentation, a feat previously out of reach.


Overall, our main contributions are as follows:
\begin{itemize}
    \item We first provide a benchmark for unsupervised video semantic segmentation and compare existing SotA self-supervised models' performances \str{Is this our strongest contribution to put as a first one? I would say that our main contribution is the insight that ``In the context of self-supervision, we are the first to show that videos should not be viewed as simply a stack of images that could be replaced by even bigger image datasets; rather, they play a critical role in the generalization of representation learning on visual observations due to their much broader diversity''. Or something like that}
    \item We propose a novel method~\methodabbrev~for dense self-supervised segmentation and demonstrate its ability to learn from the temporal signals present in videos %
    \item We extensively ablate the presented method and highlight the sources of gain \str{Is that a contribution? I would call it a minimum requirement for any publication.}
    \item We show that~\methodabbrev~yields state-of-the-art unsupervised semantic segmentation performances not only on videos, as would be expected, but \textit{even} with images, across datasets and evaluation protocols.
\end{itemize}








==> _old02_introduction.tex <==
\section{Introduction}
\cs{First paragraph is unfocused. What is the goal of this paper, what is the problem statement, what have others done to reach that goal/solve the problem, what will we be doing differently/novel?}
Dense self-supervised learning, whereby  meaningful deep features for each pixel or patch of input are learned in an unsupervised manner, has recently received increasing attention~\cite{ziegler2022self, henaff2021efficient, van2021unsupervised, seitzer2022bridging}.
\cs{Empirical results and state-of-the-art are for the experiments, not for the opening paragraph trying to explain an intellectual contribution.}
Motivated by empirical results that demonstrate performance gains in particular for dense downstream tasks such as object segmentation and detection~\cite{henaff2021efficient,purushwalkam2020demystifying}, advances in this field have also pushed the state of the art in unsupervised semantic segmentation performance remarkably.
\cs{This could be relevant related work that has the same goal? But not clear currently.}In particular, recent works such as STEGO~\cite{hamilton2022unsupervised} and  Leopart~\cite{ziegler2022self} have demonstrated the potential of successfully adapting image-pretrained Vision Transformers for this task.



\cs{What is the function of this paragraph for the reader, I get some details but the high-level idea of the paper and its novelty has not been sold yet, and I am not convinced the text below is critical for understanding the paper.}
This was accomplished mostly be generalising image-level self-supervised tasks to the spatially dense domain: Given an image $I$, and an augmented view $I'$ utilize the correspondence between these two to learn spatial features. 
In the case of a color augmentations, this correspondence is simply given by the identity. 
For cropping augmentation,  feature similarity can be simply imposed on the overlapping parts either by aggregating~\cite{henaff2021efficient,henaff2022object} or by matching RoIs~\cite{ziegler2022self}. 

\cs{Why is switching the modality of interest? Motivation is not clear to me.}
In contrast to these works, in this paper we are interested in learning from video data.
Unlabelled videos, which are abundantly available, are an as-of-yet mostly untapped source for unsupervised learning of image models. 
While some non-dense works~\cite{gordon2020watching, kipf2021conditional} assumed the passage of time  as a type of image augmentation, these works have generally reported reduced performances even when compared to simple image-based pretraining methods, highlighting the shortcomings of such assumptions.  In contrast, we believe that the additional time-dimension requires explicit modelling and can be used to obtain much richer unsupervised visual understanding. To this end, in this paper we address challenge of learning dense representations from video data.
The main challenge arises from  the additional temporality of video data:
When comparing two frames with each other, it is not clear which pixels should retain similar embeddings and which should not, due to possible object, camera and background motion between the frames. 
Learning from videos therefore introduces the additional necessity to \textit{learn the correspondences}, leading to a chicken-and-egg problem, where the correspondences are required for learning dense features -- which in turn enable good correspondences. 

Our first contribution is to provide a solution to this problem, by designing two separate modules that tackle the correspondence and the dense learning, respectively. For the former, we introduce the Feature Forwarder (\textsc{FF}) module. The \textsc{FF} leverages the good tracking performance of pretrained image models, such as DINO~\cite{caron2021emerging}, and allows us to infuse the model with temporal consistency, further tuning it. 
On top of this, we introduce a spatio-temporally dense clustering module, which learns unsupervised clusters across samples, locations and time. Using these two components and starting from image-pretrained features, our proposed method allows \textit{timetuning} (\methodabbrev) the dense representation in a self-supervised manner. 

Our second contribution is to provide comprehensive evaluation protocols to test the performance of state-of-the-art dense self-supervised learning models in the image domain on three video semantic segmentation datasets. Our experiments show the performance of such models significantly degrades when evaluating them on videos. 
Even fine-tuning the models on video data does not increase performance, due to insufficient modelling of temporal variation that can arise from object, background or camera motion. In contrast, our method consistently achieves state-of-the-art performances not only for the task of unsupervised semantic segmentation of videos, but also for \textit{image} semantic segmentation, a feat previously out of reach for methods trained on videos.






\begin{figure*}[!t]
    \centering
    \includegraphics[width=2.0\columnwidth]{Images/TimeT.pdf}
    \caption{\textbf{\methodname~overview.} We conduct self-supervised video semantic segmentation by tuning image-pretrained models with temporal information from videos. \textbf{(a)}: Our general pipeline of adapting an image-pretrained ViT transformer on video data using our dense clustering loss. \textbf{(b)}: Detailed view into our Feature Forwarder module that is used for aligning cluster-maps from past frames to logit-features of future ones. Our method obtains state-of-the-art unsupervised semantic segmentation performances on videos \textit{and} images. }
    \label{fig:schematic}
\end{figure*}


==> _old03_introduction.tex <==
\section{Introduction}
Dense self-supervised learning, whereby  meaningful deep features for each pixel or patch of input are learned in an unsupervised manner, has recently received increasing attention~\cite{ziegler2022self, henaff2021efficient, van2021unsupervised, seitzer2022bridging}. Recently, STEGO~\cite{hamilton2022unsupervised} and Leopart~\cite{ziegler2022self}, two state-of-the-arts of the field, have shown that the models trained in a dense self-supervised way can considerably improve the performance of downstream tasks such as object detection~\cite{henaff2021efficient,purushwalkam2020demystifying}, and unsupervised semantic segmentation. However, as we will show empirically, such models that are trained on images struggle to achieve a similar performance when they are tested on video datasets for the same task. Also, The problem is not solved even after fine-tuning such models on video datasets. One reason for the problem is that such models are not explicitly trained to provide consistent segmentation maps for different frames of a training video, which results in higher per frame segmentation scores compared to per clip and per dataset numbers. In this paper, we focus on providing a dense self-supervised learning model that learns from videos to enhance its features and better align itself with temporal dynamics.

Our first contribution is to evaluate the performance of state-of-the-art image models on videos. Since there is no previous work in the unsupervised video semantic segmentation, inspired by the image domain \cite{ziegler2022self}, we introduce per frame, per clip, and per dataset evaluation protocols that can better show the capabilities and limitations of such models on videos. As videos are one of the dominant learning signals for human, it seems critically important to have an insight over the performance of different models in this domain as well. As mentioned previously, our results show image-based models have trouble getting the same performance on videos and usually contain the object-centric bias of the image datasets, which might explain their worse performance even during their fine-tuning on videos.



To address the issues, learning better features directly from videos is one possible solution; however, as also indicated by~\cite{jabri2020space}, this usually leads to a chicken-and-egg problem, where the correspondences are required for learning dense features -- which in turn enable good correspondences. In the image domain, methods usually make use of augmentation and image-specific biases to find the correspondence between different inputs.  This is accomplished mostly be generalizing image-level self-supervised tasks to the spatially dense domain: Given an image $I$, and an augmented view $I'$ utilize the correspondence between these two to learn spatial features.  In the case of color augmentations, this correspondence is simply given by the identity. For cropping augmentation,  feature similarity can be simply imposed on the overlapping parts either by aggregating~\cite{henaff2021efficient,henaff2022object} or by matching RoIs~\cite{ziegler2022self}. Following the same way, some non-dense works~\cite{gordon2020watching, kipf2021conditional} assumed the passage of time  as a type of image augmentation; yet, these works have generally reported reduced performances even when compared to simple image-based pretraining methods, highlighting the shortcomings of such assumptions.  In contrast, we believe that the additional time-dimension requires explicit modelling and can be used to obtain much richer unsupervised visual understanding.

To this end, in our second contribution, we address the main challenge that arises from the additional temporality of video data: When comparing two frames with each other, it is not clear which pixels should retain similar embeddings and which should not, due to possible object, camera and background motion between the frames. We propose two separate modules to tackle the correspondence and the dense learning, respectively. For the former, we introduce the Feature Forwarder (\textsc{FF}) module. The \textsc{FF} leverages the good tracking performance of pretrained image models, such as DINO~\cite{caron2021emerging}, and allows us to infuse the model with temporal consistency, further tuning it. 
On top of this, we introduce a spatio-temporally dense clustering module, which learns unsupervised clusters across samples, locations and time. Using these two components and starting from image-pretrained features, our proposed method allows \textit{timetuning} (\methodabbrev) the dense representation in a self-supervised manner. our method consistently achieves state-of-the-art performances not only for the task of unsupervised semantic segmentation of videos, but also for \textit{image} semantic segmentation, a feat previously out of reach for methods trained on videos.
  






\begin{figure*}[!t]
    \centering
    \includegraphics[width=2.0\columnwidth]{Images/TimeT.pdf}
    \caption{\textbf{\methodname~overview.} We conduct self-supervised video semantic segmentation by tuning image-pretrained models with temporal information from videos. \textbf{(a)}: Our general pipeline of adapting an image-pretrained ViT transformer on video data using our dense clustering loss. \textbf{(b)}: Detailed view into our Feature Forwarder module that is used for aligning cluster-maps from past frames to logit-features of future ones. Our method obtains state-of-the-art unsupervised semantic segmentation performances on videos \textit{and} images. }
    \label{fig:schematic}
\end{figure*}


==> _old_03_method.tex <==
{\color{gray}
\section{Proposed Method}




We propose a temporal fine-tuning operator, which can be used to make pre-trained models, trained solely on images, temporally consistent. Since a dense segmentation task is addressed, we employ a pre-trained ViT \cite{dosovitskiy2020image} that has been shown to keep the spatial relationship of input patches in the final patch representations \cite{caron2021emerging}. Similar to recent works in the image-domain such as Leopart \cite{ziegler2022self}, we try to fine-tune the patch representations to contain object part information, which can be used in the further down-stream segmentation task. To do the fine-tuning, we force the representations of different views of an input image to be highly similar across time. However, detecting different views of the same objects in different frames is not trivial \cite{jabri2020space}. To address this issue, we use the temporal smoothness aspect of videos and assume each spatial location or patch in the input space can only move in a local window around itself. Therefore, the most similar patch-representations in a local window of different frames are assumed to represent equal contents. This means, given a  decent patch representations obtained from pre-trained networks, by tracking patch locations in the local windows of temporally close frames different object views can be detected across time. Having found different views of the same object, similar to the existing self-supervised learning trend, we train an MLP head to make their representations not only be locally the most similar ones but also globally across the whole training set. To address this issue, we use a self-supervised approach called SwAV \cite{caron2020unsupervised} yet on the patch representations instead of image-representations. We show in this way, the 


\subsection{Background}
Our method exploits image representations extracted by a vision transformer. In this part, we explain the components that have been used and will go through the detail in the next part.

\paragraph{Vision Transformers.} Vision transformers \cite{dosovitskiy2020image} operate on a sequence of patches of fixed size $P\times P$. For a color image $I$ of spatial size $H \times W$, we have $N=\frac{H \times W}{P^2}$  patches of size $P^2$ (we assume for simplicity that $H$ and $W$ are multiples of $P$). Each patch is first embedded in a $d$-dimensional latent space via a trained linear projection layer. An additional, learned vector called the ``class token'', CLS, is adjoined to the patch embeddings, yielding a transformer input in $R^{(N+1)d}$.  In this paper, in spite of classification that only uses the CLS token, we employ all $N$ features of the final layer. The features can be selected from either $Q$, $K$, or $V$ values from the last self-attention block.

\paragraph{Sinkhorn-Knopp Assignment Algorithm.}
The algorithm tries to solve the optimal assignment problem using an iterative approximation. In our case, we are looking after finding the optimal assignment between our spatial patches and a set of prototypes. The similarity measure is cosine similarity and the number of iteration is set to three. The main benefit of the Sinkhorn-Knopp algorithm is keeping the entropy of assignment between the patches and prototypes to a given minimum threshold, which avoids getting into trivial solutions and mode collapse. More details can be found in \cite{knight2008sinkhorn}.


\subsection{Method}


\paragraph{General idea for images.}
Consider $I_1$ and $I_2$ as two arbitrary training samples, from which the feature maps $F_1$ and $F_2 \in R^{D \times \frac{H}{P} \times \frac{W}{P}}$ are extracted. Also suppose the feature extractor is ViT. Intuitively, if there exist any relationship between specific regions of $I_1$ and $I_2$, then the same relationship should also hold for the extracted features of the corresponding regions. This approach has been generally used by the previous methods such as Leopart \cite{ziegler2022self}, except $I_1$ and $I_2$ are not picked randomly but represent different views of the same input. Therefore, $I_2$ can be shown as a function of $I_1$, \ie, $I_2{=}A(I_1)$. This means, the same relationship should also exist between $F_1$ and $F_2$, leading to the same patch representation for the intersection of different views of an input image. Also, to prevent the representations from collapsing or getting stuck in the same values for all different inputs, Sinkhorn-Knopp Assignment is used. It has been shown the learned features are more generalizable for down-stream semantic segmentation tasks. Here, we are going to follow an entirely different approach yet with the same intentions. Instead of using augmentations to generate different views of an input image, we aim to use natural augmentations existing in unlabeled videos. 



\paragraph{Our innovation for video data.} In videos, we do not know the exact relationship between frames: we do not know if an object has moved or hasn’t moved, a-priori.


In addition, as we are conducting spatially-dense training, we need a way to map one patch in $F_1$ to another one in $F_2$. To this end, we propose the Temporal Patch Propagator (TPP) that finds the correspondence of patches between two frames according to the following (see Algorithm 1 for details): 

\begin{enumerate}
    \item Neighborhood assumption. Given two temporally close frames $I_1$ and $I_2$, each patch of $I_1$ can only move to a local window around it in $I_2$ since the frames are changing smoothly across time.
    
    \item Semantic similarities indicate movement. If the respective feature maps $F_1$ and $F_2$ are of good quality then for two patches $p_{(1,i)} \in F_1$ and $p_{(2,j)} \in F_2$ in a local window (see a)) are likely to represent the same semantic content if their similarity exceeds a certain threshold. This means, similarities from feature maps can be used to compute a function that maps every patch from frame 1 to patches in frame 2.
\end{enumerate}



\paragraph{Propagator.}

\paragraph{Implementation.} We start from a pre-trained self-supervised backbone, \eg, DINO \cite{caron2021emerging} to extract  $F_1$ and $F_2$, then to find the equivalent of $p_{(1,i)}$ in $F_2$, a local window around this location is used to determine which location(s) is consistent with our first and second assumptions. 

After finding the matching patches in different frames, the next goal is to make the representations similar. This provides the training signal. Note that while the representation of equal patches might be similar in a local window, they might not be similar globally. To address this issue, we use a self-supervised clustering approach also used in SwAV \cite{caron2020unsupervised}, yet on the patch representations of frames instead of the image-level representations as the original method does. 



Then $\text{C-Map}_1$ is passed to the Sinkhorn-Knopp algorithm to craft the optimal assignment  $\text{SK-Optimal}_1$. Next, $\text{SK-Optimal}_1$ is propagated by TPP to the last frame where it is compared with $\text{C-Map}_T$ using a cross entropy objective function: 
\begin{align}
        \text{C-Map}_{T}(i, j) = <F_T(i), Pr_j>, \forall i \in N\\
        \text{C-Map}_{T}(i, j) = \frac{e^{\text{C-Map}_T(i, j)/\tau}}{\sum_j e^{\text{C-Map}_T(i, j)/\tau}}\\
        \text{Loss} = \sum_{i,j} \text{P-Map}_1(i, j)\log(\text{C-Map}_T(i, j))
\end{align}
where the first equation computes the similarity of each patch representation with each of the prototypes, and the second equation normalizes the cluster maps with Softmax normalization. This forces the patch representations of different frames to not only be locally consistent but also globally. Fig. 1 shows an overview of our method and Fig. 2 shows the TPP algorithm in more detail. 


\subsection{Benchmarking Pipeline}
Despite image domain, there is no benchmark on unsupervised semantic video object segmentation. Therefore, we propose the first benchmark on videos and introduce three evaluation protocols that are specific to video domain requisites. Given a trained object segmentation model, the first one is that different objects in a frame should be assigned different IDs, which is similar to the image domain. The second one is that the assigned class IDs to different objects must be consistent over time, which is an inherent characteristic of videos, since the frames are not independent. The third one that can be seen as an extreme combination of the first and the second requisites is that the assigned IDs should be globally different yet consistent across the training dataset. We call the first, second, and third approaches \textit{frame-wise}, \textit{clip-wise}, and \textit{dataset-wise} evaluation metrics, respectively.

In order to assign class IDs, followed by the trend in the image domain, we apply K-Means on the representation of the given pre-trained model to produce a cluster map for each input data. Then, the cluster maps are matched to the test-time ground truth and their MIOU is reported. Therefore, given an input data with the size [batch-size, clip-size, c, h, w], the Model $M$, the matching algorithm $MA$, and the clustering algorithm $C$, Algorithm \ref{algorithm:benchmark} shows  each of the mentioned evaluation metrics.




}
